Towards Personalized Explanation of Robot Path Planning via User Feedback

Prior studies have found that explaining robot decisions and actions helps to increase system transparency, improve user understanding, and enable effective human-robot collaboration. In this paper, we present a system for generating personalized explanations of robot path planning via user feedback. We consider a robot navigating in an environment modeled as a Markov decision process (MDP), and develop an algorithm to automatically generate a personalized explanation of an optimal MDP policy, based on the user preference regarding four elements (i.e., objective, locality, specificity, and corpus). In addition, we design the system to interact with users via answering users' further questions about the generated explanations. Users have the option to update their preferences to view different explanations. The system is capable of detecting and resolving any preference conflict via user interaction. The results of an online user study show that the generated personalized explanations improve user satisfaction, while the majority of users liked the system's capabilities of question-answering and conflict detection/resolution.

==> draft/0_abstract.tex <==
 With the development of technologies like autonomous driving and interactive robotics, the number and diversity of users affected by autonomous decision-making systems will rise. However, the average user has little understanding of how decisions are made. Explainable AI, or xAI, works to combat this issue by providing explanations about system behavior. Research suggests that explanations are social entities that should adapt based on user and situation. So, this paper develops an approach to generate feedback-based explanations and feedback-based question-answers personalized to a user while resolving any potential user preference conflicts that are created. We present a system to automatically generate these personalized explanations and answers as well as formalize the definition, detection, and resolution of different types of user preference conflicts. The results of a user study evaluating these methods with 88 participants on Amazon Mechanical Turk shows that users prefer preference-based explanations, but the inclusion of preferences does not increase user understanding. Additionally, our study shows that user preferences do not increase the understanding or satisfaction of question answers and that our conflict resolution approach is both understandable and satisfying.

==> draft/1_Intro.tex <==
\begin{comment}

\todo{The introduction should very clearly describe: \\
- what's the problem? motivate it well using concrete examples. \\
- what's the state of the art? what's the gap? \\
- what are the challenges? \\
- a summary of our approach with justifications. \\
More specifically to this paper, we need to articulate very clearly: \\
- why explanations? what do we mean by explanations? \\
- why feed-back based (to be distinguished with our IROS paper)? \\
- what conflict? where it comes from? why it is a challenge?
}

From GPSs to workplace schedulers, autonomous decision-making systems are becoming a part of our daily lives. However, the average lay-user struggles to understand how these systems make decisions, leading to possible misunderstanding, mistrust, and misuse \cite{goebel2018explainable}. Thus xAI, or explainable AI, has expanded rapidly to provide users an explanation of the system's actions. Currently, state-of-the-art systems focus on building an approximate model of the more complex decision-making functions, generating interpretable explanations of the system’s behavior \cite{arrieta2020explainable,Gunningeaay7120,Mittelstadt2019}. However, not all xAI systems take the user's preferences into account, generating the same basic explanation for all users \cite{Kraus2020AIFE}. Research suggests that explanations are social entities and humans prefer the ability to adapt explanations by situation \cite{miller2017explanation}. This adaptive nature allows for the individualization of explanations and thus the increase of understanding on a person-to-person basis. Yet, adaptation comes with a significant price. Each user needs their own personalized explanation and if a user's preferences change there could be a conflict present within them. A naive answer would generate a basic explanation of system actions or disregard preferences that cause conflicts. However, this may cause the user to become confused as to how their preferences are being used and why only some of their preferences have been met, placing further burden on the user.

This paper develops an approach to generate feedback-based explanations and feedback-based question-answers while accounting for potential user preference conflicts and resolving them. Primarily, we focus on choosing specific structured language templates to create feedback-based explanations specific to the user and answer the user's further questions in a personalized way. Moreover, we work to identify conflicts present and provide solutions to the user before they are set in the system and cause additional issues. This way we know the system provides an understandable and satisfying explanation or answer to the user.
 
 \begin{figure}[ht]
     \centering
     \includegraphics[width=0.6\linewidth]{Figures/Grid.png}
     \caption{An example grid map for robotic planning. Green grids: start (S) and destination (D). Black grids: buildings. Red grids: dead-ends. Yellow grids: urban roads. White grids: highways. }
     \vspace{-10pt}
     \label{fig:grid}
 \end{figure}
 
  \startpara{Motivating Example} Consider the situation. A robot plans to move through the grid shown in Figure 1 to deliver a package to a user. The user wants the robot to take the blue route to minimize the amount of risk and report the largest amount of information about its route in an explanation. However, at state 17 an accident occurs and the robot is slowed down considerably. Now the user wishes to change the robot's objective to minimize the amount of time that the trip will take and have it only report the most important information. The user's preferences have changed. A naive approach would pass the user's new preferences to the robot and allow it to continue, but this approach disregards the user's preferences or possible preference conflicts. The robot itself would be unable to resolve these issues. Therefore, we create a feedback-based explanation or question-answer specifically tailored to the user's wants. In the event of a conflict, we inform the user of the detected change and confirm that the user has correctly input their preferences. We explain any conflicts and possible resolutions. This way, the user can make an informed decision that satisfies their needs and can be fulfilled by the system.
 
 \startpara{Contributions}
 We summarize the major contributions of this paper as follows:
 \begin{enumerate}
    \item A formalization of feedback-based explanations using several common user feedback measures
    \item An investigation of user interaction to detect and resolve user feedback conflicts
    \item A presentation of potential explanations to increase user understanding of those detected conflicts and resolutions
    \item An Amazon Mechanical Turk user study to evaluate the effectiveness of feedback-based explanations in terms of user understanding and satisfaction
\end{enumerate}
\end{comment}

With the development of technologies such as autonomous driving and interactive robotics, the number and diversity of users affected by autonomous decision-making systems will rise. However, the average lay-user struggles to understand how these systems make decisions, leading to possible misunderstanding, mistrust, and misuse \cite{goebel2018explainable}. Thus, xAI, or explainable AI, creates simplified interpretable models as approximations of complex decision-making functions to generate basic understandable explanations of the system’s behavior. \cite{arrieta2020explainable,Gunningeaay7120,Mittelstadt2019}. However, many xAI systems do not effectively consider the user’s preferences when providing information, generating the same basic explanation for all users \cite{Kraus2020AIFE}. Research suggests that explanations are social entities and humans prefer the ability to adapt explanations \cite{miller2019explanation} as well as have a diverse set of preferences regarding explanation overall \cite{feng2018contrastive}. Thus, by creating a personalized explanation of the system’s behavior based on the user’s preferences and feedback we can decrease possible misunderstanding and increase user satisfaction. Furthermore, if a user's preferences are used by the system, such as in \cite{VelosoVerbalization}, the effects of the preferences given are not often evaluated before being set. This can lead to conflicts within the preferences themselves or between the preferences and the environment depending on the effects caused.

\begin{comment}
Consider this situation. A robot is currently located at state \revise{12} in Figure 1 as it tries to deliver a package to a user, but an accident has occurred, slowing down the robot considerably. The user now prefers that the robot take the shortest path and also take only the safe highways and ignore risky alleyways. Based on the user's new feedback, we can update the robot's actions and the explanation that we provide. However, there is an obvious conflict as the shortest path, shown in red, does not contain only highways. A naive answer would generate a basic explanation of system actions and disregard preferences that cause conflicts. However, this may cause the user to become confused as to how their preferences are being used and why only some of their preferences have been met, placing further burden on the user. How should we determine if there are any issues with the user’s preferences and then proceed to update a possible explanation?
\end{comment}

\revise{
Consider the following situation. A user is trying to plan a robot’s route from start (S) to destination (D) through Figure 1 so that it can deliver a valuable package. Originally, the user wishes the robot to take the shortest possible route and report only the most important information to minimize delivery time. However, before deployment the user changes their mind and now prefers the robot take the safest path instead and report its actions as it passes through any risky highways. The user has now updated their planning preferences. Based on the user’s new feedback, we should update the robot’s actions and the explanation of them that we provide. 
Yet, how should we do this update and how do we determine if the robot can actually fulfill the user’s wants? A naive approach would be to generate a basic readout of the robot’s path, disregarding any preferences that cause conflicts. However, this may cause the user to become confused as to how their preferences are being used and why only some of their preferences have been met, placing further burden on the user.}


\begin{figure}[ht]
     \centering
     \includegraphics[width=0.6\columnwidth]{Figures/Grid.png}
     \caption{A map for robotic planning. Blue: start (S) and destination (D). Black: buildings. Red: risky road. White: safe road. Star: landmark}
     \vspace{-10pt}
     \label{fig:grid}
 \end{figure}

Creating these feedback-based explanations comes with significant challenge. First, each user needs their own personalized explanation, placing significant burden on the system. Second, a user’s preferences could contain some sort of conflict. As a user’s preference change, there becomes more potential for these types of conflicts to occur as the user may not fully understand what is possible for the system or environment. Thus, we must balance the user’s satisfaction with system performance.

\begin{comment}
\begin{figure}[ht]
     \centering
     \includegraphics[scale=0.4]{Figures/Grid.png}
     \caption{An example grid map for robotic planning. Green grids: start (S) and destination (D). Black grids: buildings. Red grids: dead-ends. Yellow grids: urban roads. White grids: highways. }
     \vspace{-10pt}
     \label{fig:grid}
 \end{figure}

Consider this situation. A robot plans to move through the grid shown in Figure 1 to deliver a package to a user. The user wants the robot to take the safest route and report a large amount of information. However, at state 17 an accident occurs, and the robot is slowed down considerably. Now the user wishes to take the shortest route and only report the most important information. The user’s preferences have changed. How should we determine if there are any issues with the user’s preferences and then proceed to update a possible explanation?

A naive answer would generate a basic explanation of system actions and disregard preferences that cause conflicts. However, this may cause the user to become confused as to how their preferences are being used and why only some of their preferences have been met, placing further burden on the user. 
\end{comment}
This paper develops an approach to generate feedback-based explanations and resolve any potential user preference conflicts. Primarily, we focus on choosing specific structured language templates to combine to create an overall personalized explanation to remove burden on both the system and the user. Moreover, we work to identify conflicts present using basic logical rules and provide solutions for user selection. Using logical rules allows for our preference conflict detection approach to be expanded and applied generally based on the available preferences. Moreover, having the user to choose their desired resolution to a conflict allows us to provide the most understandable and satisfying answer to the issue for each user.

 \startpara{Contributions}
 We summarize the major contributions of this paper as follows:
 \begin{enumerate}
    \item A prototype type system to produce feedback-based explanations, generate question-answers and resolve any possible user preference conflicts through user interaction
    \item A formalization of the definition, detection, and resolution of different types of user preference conflicts
    \item An evaluation of feedback-based explanations, feedback-based question-answers, user preference conflict detection and resolution approaches
\end{enumerate}


\begin{comment}
    \begin{itemize}
    \item User Preferences in Explanation
    \begin{itemize}
    \item Explanations as Social Entities - Miller's Work
     \item Explanation Preference Factors - Veloso and Surrounding Papers
     \item Challenges of User Preference Explanations - Sarrit 
\end{itemize}
  \item Conflict Detection
   \begin{itemize}
    \item Social Media - Detect When There is a Discrepancy Between Share Settings of Users
    \item Recommendation System - When an Item is not Available Matching All Wants
    \item Explanations - No Work in Detection Conflicts in the Explanations Themselves
\end{itemize}
  \item Conflict Resolution
  \begin{itemize}
    \item Social Media - Setting Security Preferences to Please All Parties
    \item Recommendation System - Recommending Products Most Close to Preferences or Recommending Next Preferences to Search
    \item Explanations - How to Present Preferences that Do and Do Not Match Products
\end{itemize}
\end{itemize}
\end{comment}

\startpara{Related Work} Although many autonomous decision-making systems collect some aspect of user preferences, for example, recommendation systems, most systems do not utilize this information
to better explain their decisions instead using them to better the system's performance \cite{LearningSystem,Iaco2019LearningAL,Li2020SeamlesslyUA}. 

However, the importance of providing explanations is based in the social sciences with works such as \cite{miller2019explanation,madumal2019grounded} supporting the usage of adaptable or social explanations to increase user understanding, especially those with multiple diverse users \cite{Kraus2020AIFE}. Generating explanations for AI-based decision-making systems deals significantly with the balance between system accessibility and system performance \cite{feng2016synthesis}, and by balancing these trade-offs, we are able to increase system interpretability \cite{Lieaay6276}.  So, when generating an explanation, we need to carefully choose (or allow the user to choose) as many explanatory factors as possible to increase user understanding and decrease user burden. 

Some systems create personalized explanations based on user preferences \cite{VelosoVerbalization,Veloso2}, or create explanations using structured language templates \cite{feng2018counterexamples,Hayes10.1145/2909824.3020233}. Yet, most of this work is theoretical with little practical evaluation being performed. Additionally, none of these previous works present contrastive explanations (why an event $P$ happens instead of some event  $Q$) to users even though social science points to these types of explanations increasing user understanding and user satisfaction more than other explanation types\cite{miller2019explanation,feng2018contrastive}.

Finally, previous work in robotic planning does not address the possibility of conflicts or further user questions. However, social media and recommendation systems have looked at the possibility of conflicts regarding user preferences. Social media preference conflicts occur when users disagree over preferences such as a post's share settings and are easily resolved by following one user's preference based on the situation \cite{SocialMediaConflicts,SocialMediaConflicts2,SocialMediaConflicts3}. Recommendation system conflicts arise when no product or action matches a user's preferences and resolution occurs by explaining why a choice is shown or recommending a new preference to set \cite{RecommendationSystemConflicts,Pu2008UserInvolvedPE}. Still, there has been little work to detect conflicts within the user preferences themselves, especially in robotic planning systems, as these types of personalized explanation conflicts are often more complex, involving multiple preferences and possibly resolving in an unsatisfying way.


==> draft/3_Preference.tex <==
\subsection{Adapting Explanations to Fit User Preferences}

\begin{figure}[!h]
  \centering
    \includegraphics[scale=0.55]{Figures/OverallFlowChart.png}
  \caption{Connections within the User Preference Feedback System}
\end{figure}

\begin{comment}
\begin{figure}[!h]
  \centering
    \includegraphics[scale=0.5]{Figures/UserInterface.png}
  \caption{UI for a User Preference Feedback System}
\end{figure}
\end{comment}

\begin{comment}
\todo{Start this approach section with an brief overview paragraph to describe the overall flowchart without going into details (focusing on the flow and input/output of different blocks), then each subsection corresponding to a major block in the flowchart. We should also show the user interface figures, to make it more concrete.  }
\end{comment}

In this section, we define a system, shown in Figure 2, that produces a feedback-based explanation. Users begin by choosing their desired explanation and route preferences for a presented map using drop down boxes in the UI. These choices are then set in a tuple for reference later and then used to generate an explanation regarding the actions of the system. Once the explanation is presented, the user now can ask further questions if needed. For each additional question that is asked we create an additional explanation based on the user’s preferences to answer that question. When the user has no further questions, indicating it using a "Next Position" button in the UI, we check to see if the user has updated their preferences at this time and if there are conflicts present in those preferences. No conflict present causes the system to move forward, while the presence of a hard or soft conflict causes us to react accordingly either confirming the users preferred preferences or resolving any potential issues through user interaction. The chosen preferences are then set and the position is updated.

\begin{comment}
\begin{figure*}[!h]
  \centering
    \includegraphics[scale=0.25]{Figures/UserInterface.png}
  \caption{Example of User Interface to Provide Explanations Based on User Preferences}
  \label{fig:overallChart}
\end{figure*}
\end{comment}

\begin{comment}
\begin{figure*}
     \centering
     \begin{subfigure}[]{0.25\textwidth}
         \centering
          \includegraphics[scale=0.25]{Figures/UserInterface.png}
            \caption{Example of User Interface}
         \label{fig:userInterface}
     \end{subfigure}
     \hfill
     \begin{subfigure}[]{0.42\textwidth}
         \centering
         \includegraphics[scale=0.37]{Figures/DoubleTable.png}
     \caption{Explanation Preference Options and Further Questions}
     \vspace{-10pt}
     \label{fig:table2}
     \end{subfigure}
    \caption{User Interface for User Preference Feedback System}
\end{figure*}

Our system uses four user preferences: objective (route type), abstraction (explanation subject), locality (route section of interest), and specificity (level of information). Objective refers to the objective that the system currently has to accomplish such as finding the shortest distance or most flexible path. Regarding explanations, the objective effects the reasoning that should be provided for the choices presented. According to \cite{VelosoVerbalization,DeyAbstraction}, “Abstraction varies the vocabulary and concepts used in the narrative form concrete robot concepts, such as distances, speed, and time to abstract concepts, such as hallways, room, and landmarks.” Locality “varies the particular parts of the experience that the narration focuses on, from the global path to a local region or a landmark of interest” \cite{VelosoVerbalization,TomasonLocality}. We use the three levels of locality defined above with a global explanation presenting an explanation of all states, a regional explanation presents an explanation for several states, and a landmark explanation presenting an explanation of one state. Specificity “varies the total number of concepts or words used” \cite{VelosoVerbalization,bohus2014directions}. For our system, varying the specificity varies the user-defined $\alpha$ when calculating the critical states present in the MDP [19]. This effects where the user may update the system and receives an explanation. Figure \ref{table:preftable} shows the options avalible to users in o
\end{comment}

Our system uses four user preferences: abstraction (explanation subject), locality (route section of interest), specificity (level of information), and  objective (route type). According to \cite{VelosoVerbalization,DeyAbstraction}, “Abstraction varies the vocabulary and concepts used in the narrative form concrete robot concepts, such as distances, speed, and time to abstract concepts, such as hallways, room, and landmarks.” Locality “varies the particular parts of the experience that the narration focuses on, from the global path to a local region or a landmark of interest” \cite{VelosoVerbalization,TomasonLocality}. Specificity “varies the total number of concepts or words used,”\cite{VelosoVerbalization,bohus2014directions}. Specifically, in our system, it varies the number of critical states where the actions are explained to the user \cite{Chen2020TowardsTR}. Finally, objective refers to what the system currently has to accomplish. Regarding explanations, the objective affects the reasoning provided for the actions chosen. Table \ref{table:preftable} shows the options available to users for each preference type.

\begin{comment}
\begin{figure}[ht]
     \centering
     \includegraphics[scale=0.3]{Figures/Table2.png}
     \caption{User Preference Options for System}
     \vspace{-10pt}
     \label{fig:table2}
 \end{figure}
 \end{comment}

\begin{comment}
In generating a feedback-based explanation, the user’s specificity and locality are used to determine the length of the total explanation provided. States that are not critical in terms of the set specificity or not a part of the desired locality are not presented to the user within an overall explanation as the user has not indicated an interest in them. Thus, the user is only able interact with the system at states that match their preferences, lessening the burden placed on the user. We then choose the correct structured language template for the explanation through the user’s indicated abstraction and generate the reasoning using the objective preference. Since the potential objectives vary widely, the reasoning must be chosen correctly to match the user's interests and support user understanding.
\end{comment}

\revise{
A structured language template is the base sentence that we adapt to form our explanations. We begin by choosing our desired template based on the user’s chosen abstraction. If the user has selected \textbf{directions}, we choose the following template as it informs the user only of the direction traveled:}\revise{\begin{center}The robot moves $<$action$>$ at position $<$location$>$ because it leads to the $<$objective$>$.\end{center}}

\revise{If the user instead has chosen \textbf{landmarks}, we use the following template as it focuses on the landmarks along the user’s path:}\revise{
\begin{center}The robot moves along the $<$landmark$>$ because it leads to the $<$objective$>$.\end{center}}

\revise{Additionally, we can generalized these templates to a wider set of robotic planning actions in the following way:}\revise{
\begin{center}The robot $<$action$>$ at $<$location$>$ because it supports the current objective: $<$objective$>$.\end{center}}

\revise{The above template can be instantiated by replacing action with the robot’s chosen action (Ex. moves east, moves along the highway), replacing location with the robot’s current position, (Ex. state 15, the gas station), and replacing objective with the current chosen objective (Ex. shortest path, safest path). So, we can think about the template as a function that takes a tuple (action, location, objective) as the input and outputs the
corresponding sentence.}

\revise{We then select the set of states for which we will explain. The user’s specificity determines if we will explain at all states within the path or just those critical to the policy. This allows the user to increase/decrease their level of information given about their path. The chosen locality will then limit the states to only those that the user is interested in based on the state type. Thus, allowing the user to choose specific sections of the path to receive information about. To create a longer explanation for multiple states, we add an additional template for each state linked by a sequencer such as “Then,” “Next,” or “Finally.” The pseudo-code for this process is shown in Algorithm 1.}

\begin{algorithm}[]
\KwIn{MDP $M$, Policy $\pi$, Route $R$, Preference Tuple $P$, Language Template $T$}
\KwOut{Explanation $\varepsilon$}
\begin{algorithmic}[1]
\STATE cS $\leftarrow$ findCriticalStates($M$)
\STATE $\varepsilon$ $\leftarrow$ Empty string\\
\FOR{s in $R$}
    \IF{s in ($R$ $\cap$ $lo$)}
        \IF{$sp$ != "critical" $||$  s $\in$ cS}
            \STATE Find $act$ $\in$ $A$(s) taken in $\pi$
            \STATE $act$, $loc$ $\leftarrow$ abstract($act$,$state$,$ab$)
            \STATE $Sen \leftarrow T(act,loc,ob)$\\
            \STATE $\varepsilon$ += $Sen$
        \ENDIF
    \ENDIF
\ENDFOR
\RETURN $\varepsilon$
\end{algorithmic}
\caption{Explanation Generation (Generalized)}
\end{algorithm}

\begin{algorithm}[]
\KwIn{MDP $M$, Route $R$, Preference Tuple $P$ = (ab,lo,sp,ob)}
\KwOut{Route Explanation}
\begin{algorithmic}[1]
\STATE cS = findCriticalStates(M,R,ob)
\STATE T = chooseTemplate(ab)
\STATE Exp = ""\\
\FOR{s in R}
    \IF{s in (R $\cap$ lo)}
        \IF{sp != "critical" $||$  s in cS}
            \STATE act = findAction(state,P)\\
            \STATE loc, lan = stateInfo(state)\\
            \STATE $T: (act,loc,lan,ob) \rightarrow Sen$\\
            \STATE Exp += $Sen$
        \ENDIF
    \ENDIF
\ENDFOR
\RETURN Exp
\end{algorithmic}
\caption{Explanation Generation (OLD)}
\end{algorithm}

\begin{comment}
\begin{figure}[!h]
     \centering
     \includegraphics[scale=0.37]{Figures/QuestionTable.png}
     \caption{Potential System Questions and Answers}
     \vspace{-10pt}
     \label{fig:table2}
 \end{figure}
 \end{comment}

\begin{comment}
\begin{example}
In Figure 1, assume that the user is located at position 17 has the following preferences: lefts/rights, all information, global, shortest path. The system begins by checking the specificity and locality choices. Since the state is a part of the “global” region and is within the path, the explanation will be provided to the user. The system then will choose a template matching the user’s abstraction needs: “We move right at position 17 because”. Next, we add the reasoning, “it leads to the shortest route” as this explains the system’s action, choosing to follow the shortest red route, and relates to the user’s desired objective, finding the shortest route. Thus, the provided explanation is “We move east at position 17 because it leads to the shortest route.” 
\end{example}
\end{comment}

\begin{example}
\revise{In Figure 1, assume the robot is at position 12 and the user has the following preferences: directions, all information, global, shortest path. First, retrieve the information that we need and instantiate the template with the following tuple: (moves east, state 12, shortest path). Thus, the resulting template for position 12 is “The robot $<$moves east$>$ at $<$state 12$>$ because it supports the current objective: $<$shortest path$>$. Since the locality is global and the specificity is all information, we remove no states from our possible explanation set. An additional template is appended for each state in the red route.}
\end{example}

\begin{comment}
Additionally, the user may ask several pre-determined questions and receive an answer using current system information, the user’s current preferences, and a structured language template to generate a related answer. The user may continue to ask questions to the system until they indicate that they are satisfied. This way, the user receives more information set to their specific preferences if they require it, but not so much information that it overwhelms them. By tailoring the answer to their specific preferences, the information addresses their wants or needs without the user having to make additional connections. 
\end{comment}

\revise{Additionally, the user may ask several pre-determined questions to receive further clarification from the system for any state within their explanation set. These questions are answered using further specified language templates. Below we show several question and answer template examples:}

\begin{enumerate}
    \item {\revise{Why did we $<$action$>$?}}
    \begin{itemize}
    \item{\revise{The robot $<$action$>$ at $<$location$>$ because it allows us to reach the destination and fulfill the objective: $<$objective$>$.}}
    \end{itemize}
    \item{\revise{Why did the robot not take a different action?}}
    \begin{itemize}
    \item{\revise{Not $<$action$>$ at $<$location$>$ causes the robot to be unable to fulfill the objective: $<$objective$>$.}}
    \end{itemize}
\end{enumerate}

\begin{comment}
1. We move $<$action$>$ at position $<$location$>$ because it leads to the destination.
2. We move $<$action$>$ at position $<$location$>$ because it leads to the destination.
3. You should update your route if there is a change in your preferences.
4. You may update your route when an important position is reached.
\end{comment}
\begin{comment}
1. The robot takes $<$action$>$ at position $<$location$>$ because $<$objective$>$ allows us to reach the destination in $<$reward$>$ [total/risky] spaces.
2.Taking $<$action$>$ at position $<$location$>$, then we add unneeded [distance/risk] to our route.
3.If you would like to $<$abstraction effect$>$, $<$locality effect$>$, $<$specificity effect$>$, or $<$objective effect$>$ then you should update your explanation preferences.
\end{comment}

\revise{The above templates can be instantiated by replacing action with the robot’s chosen action, replacing location with the robot’s current position, and replacing objective with the objective fulfilled or violated by taking a certain action. So, we can think about the templates as a function that takes a tuple (action, location,objective) as the input and outputs the corresponding sentence based on the question chosen.}

\begin{comment}
So, a structured language answer template $T$ is denoted by $T: (act,loc,r,ab,lo,sp,ob) \rightarrow Sen$ where $act \in Act$ is an action, $loc \in S$ is a location, $r$ is the reward for the route, $ab$ is the chosen abstraction, $lo$ is the chosen locality, $sp$ is the chosen specificity, $ob$ is the chosen objective, and $Sen$ is a sentence.w
\end{comment}



\begin{comment}
\begin{example}
The user is located at state 17 on the red route and has the following preferences: left/rights, all information, global, shortest path. They ask the system for more information, specifically “Why did we move in the state direction?” Since the user wants the system to provide the shortest route, the user receives the answer that “moving east will allow us to reach the destination in 8 states,” since distance is the factor that the user is interested in. However, if the user had chosen a different objective, then a different answer would be provided. For example, if the user had the safest path objective, then the answer provided would state that the blue path “provides a route with no risky states” since the user is more interested in the route’s risk than its distance.
\end{example}
\end{comment}

\begin{example}
\revise{The user is located at state 12 on the red route and has the following preferences: directions, all information, global, shortest path. They ask the system “Why did we move $<$east$>$?” The template is chosen and instantiated with the tuple (moves east, state 12, shortest path). The final template is "The robot $<$moves east$>$ at $<$state 12$>$ because it allows us to reach the destination and fulfill the objective: $<$shortest path$>$."
}
\end{example}

==> draft/4_DetectionandResolution.tex <==
\begin{comment}
\todo{Conflict detection and resolution can be combined into one section. Also we need to formalize the conflicts, not just list them in the table, but also in the text}
\end{comment}

As users may update their preferences if they are unsatisfied with their explanation received or to provide the system with new needs as the environment changes. Thus, conflicts may occur between new preferences or already set preferences. There are two types of potential conflicts hard and soft, each of which is presented with an accompanying explanation to maximize the user's understanding of what has occurred.

\begin{comment}
\begin{algorithm}[]
\SetAlgoLined
\KwIn{newPreference, currentPreference}
\KwOut{resolution}
\If{\textbf{conflict}}{
userChoice = Verify user preferences\\
\Switch{userChoice}{
    \Case{restartInput}{
    User chooses preferences\\
    Detect and Resolve Conflicts()\\}
    \EndCase
    \Case{currentPreference}{
    \Return currentPreference}
    \EndCase
    \Case{newPreference}{
    \If{\textbf{soft conflict}}{
    \Return newPreference
    }
    \ElseIf{\textbf{hard conflict}}{
    Generate resolution choices\\
    User chooses preferred resolution\\
     \Return resolution}
    \Else{
    \Return currentPreference}
    \EndCase
    }}
  \EndSwitch
}
\Return currentPreference
 \caption{Detect and Resolve Conflicts}
 \label{fig:detectAlg}
\end{algorithm}
\end{comment}

\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{lllll}
\hline
\textbf{Preference} & \textbf{Effect} & \textbf{Detection of Hard Conflicts} & \textbf{Detection of Soft Conflicts} \\ \hline
Abstraction & Changes the subject of the explanation & N/A & $ab \not= ab'$ \\ \hline
Locality & \begin{tabular}[c]{@{}l@{}}Changes the states in the route\\ Changes the states explained\end{tabular} & (Selected states $\cap$ Route) $\not\subseteq$ Route & $lo \not= lo'$ \\ \hline
Specificity & Increases/decreases number of update states & (Update states $\cap$ Route) $\subseteq$ Ø & $sp \not= sp'$\\ \hline
Objective & Changes the route through the map & Current route $\not=$ New preference route & $ob \not= ob'$\\ \hline
\end{tabular}%
}
\caption{Hard and Soft Conflict Detection Rules for Specific System Preferences}
\label{fig:conflictrules}
\end{table*}

\startpara{Detecting a Conflict}
A conflict is detected by comparing the user's new input preferences with their previously set preferences. If a change is found, then we say that a conflict has occurred and we alert the user. We define a user's \textbf{preference tuple} for our system as
$$P = (ab,lo,sp,ob)$$
where $ab$, $lo$, $sp$, and $ob$ represent abstraction, locality, specificity, and objective for our system. Given a policy $\pi$, $\pi$ \textbf{satisfies} $P$ if $\pi$ is compatible with every element of the preference tuple $P$, i.e.:
$$\pi \models P := (\pi \models ab \wedge \pi \models lo \wedge \pi \models sp \wedge \pi \models ob)$$
and $\pi$ \textbf{violates} $P$ if $\pi$ is not compatible with at least one element in the preference tuple $P$, i.e:
$$\pi \not\models P := (\pi \not\models ab \vee \pi \not\models lo \vee \pi \not\models sp \vee \pi \not\models ob)$$

Formally, we define a \textbf{conflict} $C$ between preferences $P$ and $P'$ as 
$$C := (P \not= P')$$
$$(P \not= P') := (ab \not= ab' \vee lo \not= lo' \vee sp \not= sp' \vee ob \not= ob')$$

where $P'$ is the user's preference at the next time step.

When resolving conflicts, the user  chooses how the system proceeds, increasing their agency. The user can choose their current preferences $P$, indicating that they did not make a mistake during input, choose their new preferences $P'$, indicating they did make a mistake, or start the input processes over if needed. This way, we know the user has correctly input their preferences before we try to resolve the conflict.

\startpara{Detecting Soft Conflicts}
A soft conflict occurs when a conflict is detected, but the system can still satisfy $P'$. Formally, given a map $M$, a \textbf{soft conflict} can be defined as
$$C \wedge \exists \pi \in Policy(M), \pi \models P’ $$

A soft conflict may appear to be a conflict, but does not cause an issue. However, we still confirm with their user that their preferences were correctly entered before preference input as it prevents additional system burden and user understanding. The accompanying explanation indicates confirmation by moving the system forward.

\begin{example}
The user is located at position \revise{12} on the red route and  has the current preferences: lefts/rights, all information, only alleyways, shortest path. The user changes their locality preference to global. We alert the user to the change and the user indicates no mistakes in their input. Since we can fulfill all preferences, a soft conflict has occurred and we move the system forward.
\end{example}

\startpara{Detecting Hard Conflicts}
A hard conflict is a conflict where the system cannot satisfy the user's new set of preferences and thus must provide an alternate resolution.  Formally, given a map $M$ a \textbf{hard conflict} can be defined as
$$C \wedge \forall \pi \in Policy(M), \pi \not\models P’ $$
Hard conflicts can occur both within preferences, a preference cannot be fulfilled at all, or between preferences, two different preferences conflict. Thus, it could require the user to balance multiple preference effects that they may not fully understand. This misunderstanding may cause users to set preferences with unintended consequences and potential issues. 
To detect a hard conflict, we must first try and create a route solely with the states that fulfill the preferences. If not possible, then a hard conflict has occurred and the user must change their preferences. Table \ref{fig:conflictrules} shows some more specific rules for the preferences used in our system. Some preferences cannot cause hard conflicts, such as abstraction, as these preferences only cause superficial changes. Once we have detected a conflict, we present it to the user and ask them to resolve it by choosing between several recommendations generated by the system. An explanation accompanies both the conflict and resolutions. By allowing the user to choose the resolution, we ensure the most  satisfactory and understandable set of realizable and valid preferences is given to the system.

\begin{example}
 Assume that the user is located at state \revise{12} on the red route and has the following preferences: left/rights, all information, only alleyways, shortest path. They change their objective to the safest route, creating a hard conflict between the user's objective and locality preferences as we must switch from our current red route onto the blue route which does not contain only alleyways. Thus, we need to report to the user that there is a hard conflict that they will need to resolve: "The choices you have chosen are invalid and we cannot fulfill all of your choices as only the shortest possible route contains only alleyways."
\end{example}

\begin{comment}
\startpara{Explaining Conflicts}
\begin{figure}[]
     \centering
     \includegraphics[scale=0.3]{Figures/DetectExp.png}
     \caption{Explanations Presented to Users For Hard and Soft Conflicts}
     \vspace{-10pt}
     \label{fig:detectExp}
 \end{figure}
 
All conflicts presented to the user are also explained to the user to increase the user's understanding of why the conflict has occurred. These explanations are presented in Figure \ref{fig:detectExp}. Conflicts and explanations are also ranked by importance for the user, with hard conflict appearing at the top of the list followed by the soft conflicts, to allow the user insight into which conflicts they should focus on resolving first.
\end{comment}

\startpara{Resolving Soft Conflicts}
Soft conflicts only appear to be conflicts and do not need user resolution. We confirm that the user has correctly input their preferences and move forward without pause.

\startpara{Resolving Hard Conflicts}
However, hard conflicts must be resolved by the user to maximize user satisfaction and understanding without fulfilling their total wants. Single preference conflicts are prioritized as their only resolution is a change in that single preference. We begin by generating all options for the conflicting preferences (single preference options for single preference conflicts or in pairs for between preference conflicts) and remove the options that still cause conflicts. The remaining options will be recommended to the user as possible choices. When all of the recommendations have been generated, we remove the overlapping recommendations, ordering them by likeness to the user's original new preference. This way, we suggest the user change the least preferences possible. An explanation is presented alongside the recommendation to increase user understanding of why the recommendation has been generated for them based on the conflict type and the preferences involved.
 
 \begin{example}
 Now, return to Example 4, a hard conflict. Starting with the locality preference, we generate all options: only current position, only alleyways, only highways, and global. We remove only highways and only alleyways since we know they conflict with the safest path objective. 
 We then do the same for the possible objectives, shortest path, safest path, and shortest and safest path, and remove all options but shortest path. Now, we generate all possible pairs of preferences: global and safest path ("closest to your new preference"), only current position and safest path ("has your new route, but lessens 
 your area of interest"), and only alleyways and shortest path ("return to your old preferences"). The recommendations are presented in the order above and accompanied by their corresponding explanations.
 
 \end{example}


==> draft/6_Experiments.tex <==


We designed and conducted an online user study to evaluate the proposed approach.  
We describe the study design here and analyze the results in \sectref{sec:results}.

\startpara{Experiment Design} 
We recruited 100 individuals with a categorical age distribution of 2 (18-24); 49 (25-34); 26 (35-49); 9 (50-64); and 2 (65+) using Amazon Mechanical Turk (AMT). To ensure data quality, we only accepted users on AMT that had a 90\% approval rate and had preformed at least 50 task previously. Additionally, we injected attention check questions periodically during the study.
\revise{After filtering out low quality answers, we end up with using data from 88 participants for the analysis.}

We instructed each user to consider a robot path planning problem in a grid map environment similar to Figure 2. Users were briefed about how the robot can move (north, south, east, west, stop) and the types of states that it may encounter (start, destination, obstacles, landmarks, corridors, etc.). We started by eliciting user preferences for all four elements (objective, locality, specificity, and corpus) by having the user choose from a drop-down list with explanation examples for each element. We then derived the user’s preference tuple and applied it to synthesize a personalized explanation for nine different grid map examples (3 states over 3 maps). Once the explanation was synthesized for a map and the questions about it submitted, the user was able to update their preferences for the next map (as many times as they liked from a drop-down) if they were not happy with the state of the provided information and continue on with these new preferences. We randomized the order of the presented explanations and the maps to counterbalance the ordering confound effect. 

\startpara{Manipulated Factors}
We manipulated one factor: explanation type. For each map, a personalized explanation (Ex: We move up because it leads to the shortest route.) with the user’s current preferences was presented alongside a basic explanation of a single statement of the robot’s choice of action without further reasoning (Ex: We move north towards the destination.) 

\startpara{Dependent Measures}.
For each explanation type, we asked users to rate on a 5-point Likert item their understanding (5 for fully understand and 1 for no understanding) and satisfaction (5 for fully satisfied and 1 for not satisfied). We then asked users to select the explanation that was more favorable to them for each map and also overall at the end of the survey. Finally, we kept track of the number of times that the user updated their preferences to modify the preference-based explanation for each of the nine maps.

\startpara{Hypotheses}
\begin{itemize}
    \item \textbf{H1:} Users will show a diverse range of explanation preferences across our four preference elements.
    \item \textbf{H2:} Personalized explanations are more understandable than basic explanations.
    \item \textbf{H3:} Personalized explanations are more satisfying than basic explanations.
    \item \textbf{H4:} Personalized explanations are more favorable than basic explanations.
    \item \textbf{H5:} Users will update their explanation preferences often.
\end{itemize}


==> draft/7_Results.tex <==


\begin{table*}[t]
\tiny
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccccc}
\hline
\multicolumn{2}{c}{Objective} &  & \multicolumn{2}{c}{Vocabulary} &  & \multicolumn{2}{c}{Locality} &  & \multicolumn{2}{c}{Specificity} \\ \cline{1-2} \cline{4-5} \cline{7-8} \cline{10-11} 
Shortest Path & 45 &  & Left and Rights & 77 &  & Global & 67 &  & All Information & 69 \\
Safest Path & 27 &  & Landmarks & 11 &  & Only Highways & 15 &  & Important Information & 19 \\
Shortest and Safest Path & 16 &  &  &  &  & Only Alleyways & 2 &  &  &  \\
 &  &  &  &  &  & Single Position & 4 &  &  &  \\ \hline
\end{tabular}%
}
\caption{User selection of preference elements options for personalized explanations }
\label{tab:preferences}
\end{table*}

\begin{figure}[t]
     \centering
     \includegraphics[width=0.95\columnwidth]{Figures/NumberOfUpdatesBar.png}
     \caption{Number of preference updates per user vs. number of users in each category.}
     \vspace{-10pt}
     \label{fig:updatefiguredraft}
 \end{figure}
 
 \begin{figure}[t]
     \centering
     \includegraphics[width=0.95\columnwidth]{Figures/ExpUnderstandingFigure.png}
     \caption{User understanding (mean and standard deviation) about basic and personalized explanations.}
     \vspace{-10pt}
     \label{fig:expfigureunderstandingdraft}
 \end{figure}

 \begin{figure}[t]
     \centering
     \includegraphics[width=0.95\columnwidth]{Figures/ExpSatisfactionFigure.png}
     \caption{User satisfaction (mean and standard deviation) about basic and personalized explanations.}
     \vspace{-10pt}
     \label{fig:expfiguresatisfactiondraft}
 \end{figure}

First, as shown in Table \ref{tab:preferences}, we observe that users in the online study selected preferences across all available options objective, locality, specificity, and vocabulary. This observation confirms our assumption that user preferences are diverse, and thus important to consider in explanations to meet user expectations. \textbf{So, we accept H1.}

To evaluate H2 and H3, we first begin by testing the normality of our responses using a Shapiro-Wilk test (Understanding:$\alpha$= 0.05, W = 0.855 , p$\leq0.000$, Skewed. Satisfaction:$\alpha$= 0.05, W = 0.870 , p$\leq0.000$, Skewed.). Finding that neither set of data is normally distributed, we employ a Friedman test (a repeated measure version of the more common Kruskal-Wallis test) \cite{daniel1990applied} to prove the statistical significance of the means of all responses between personalized and basic explanations.  For each Friedman test, we use an alpha value of 0.05 to ensure a confidence level of 95\% and assume a null hypothesis that the mean of responses for both explanation types will be statistically similar. As shown in Figure \ref{fig:expfigureunderstandingdraft}, we find that there is no significant statistical difference in user understanding between explanation types (Friedman: $\alpha$= 0.05, Q = 0.456 , p$\leq$0.500, Not Significant.). This is most likely due to both explanations having a goal of imparting all necessary information to the user and the simplicity of maps used in the study. \textbf{So, we reject H2.}

Furthermore, Figure \ref{fig:expfiguresatisfactiondraft} shows that we find that users are more satisfied with preference-based explanations than their basic counterparts (Friedman: $\alpha$= 0.05, Q = 6.365 , p$\leq$0.012, Significant.). \textbf{So, we accept H3.}

To evaluate H4, we utilize a Pearson's chi-squared test \cite{seltman2012experimental} to prove the statistical significance in the frequency of explanation selection. We assume an expected selection of 50/50 to represent a random selection of explanations by the users and assume a null hypothesis that the user selection of explanations will be random/fit our expected values. We once again use an alpha value of 0.05. When asked to choose which type of explanations they preferred, users choose the preference-based explanation 56.95\% of the time ($\chi^2$ :$\alpha$= 0.05, $\chi^2$ = 15.278, $\chi^2_c$ = 3.84, p$\leq$0.000093, Reject $H_0$.). Overall, 92.05\% indicate they prefer preference-based explanations to basic explanations ($\chi^2$ :$\alpha$= 0.05, $\chi^2$ = 62.23, $\chi^2_c$ = 3.84, p$\leq$0.00001, Reject $H_0$.). This higher level of satisfaction and favor may be caused by the perceived increase in user agency (i.e., the ability of users to make choices and act independently \cite{emirbayer_mische_1998}), since the users were able to choose the aspects of the explanations themselves. Additionally, by choosing the factors themselves, users were able to better guarantee that they would “like” the explanations more as they were able to request more/different information if they needed it, but did not have to deal with the additional burden of information if it was not required. \textbf{So, we accept H4.}

Finally, we observed a total of 178 preference updates among 88 users. Figure \ref{fig:updatefiguredraft} shows a breakdown of the numbers: 35 users chose not to update their preferences, while 53 users (60.23\% of the study group) updated their preferences at least once during the study. This indicates that most users will update their preferences to match a given route or map if the option is given and shows the necessity of allowing for the update of preferences to occur. \textbf{So, we accept H5.}

\startpara{Further Testing} 
In addition to the situation described above, at the end of the study, we gave each user the chance to use the interactive (answering further questions) and conflict detection portion of our system. First, each user was allowed to ask further questions (from a predefined list) about the personalized explanations that they received. We asked each user if overall they liked the ability to ask further questions/receive further reasoning about the robot’s actions and 82.95\% of users (73 of 88) stated that they did like this ability. 
Then each user was given 3 example preference conflicts, one soft (locality updated from only highways to only alleyways), one hard (shortest path updated to safest path), and one none (no updates), to resolve using the process described in our approach. We asked each user if they liked the preference conflict resolver and 93.18\% of users (82 of 88) stated that they did. Further testing will need to be done to support the use of these abilities over other possible explanation options.







==> draft/8_Conclusion.tex <==
\begin{comment}
\begin{itemize}
\item Conclusions
\item Future Work
\begin{itemize}
    \item Multi-User Explanation
    \item Update States
    \item Predicting User Resolution Choice
    \end{itemize}
\end{itemize}
\end{comment}

\revise{In this paper, we develop an approach to generate personalized explanations while resolving any potential user preference conflicts that are created. A user study with 88 participants on the Amazon Mechanical Turk platform shows that users prefer personalized explanations, but the inclusion of preferences does not increase user understanding. Additionally, our study shows that users understand and are satisfied with both our presented question answers and the conflict resolution process. In the future, we plan to further investigate methods of expanding possible user questions, creating a multi-user personalized explanation generation system, and automating the process of resolution generation.}

==> draft/_Preliminaries.tex <==
\todo{Not sure if we need a separate prelim section. I think it's more important to have an approach overview section, present the flowchart to give readers a big picture of what we're trying to do. The definitions of OBSL elements and verbalization space can be introduced in the appoach section when it is used first time. Not even sure if we need to mention MDPs in this paper, because this is a general approach that does not depend on MDPs. }

In this section, we provide the needed background for the work being presented.
\begin{comment}
We begin by providing the necessary background on Markov decision processes (MDPs) and then by defining several of the most common explanation preferences.
\end{comment}

\startpara{MDP} 
MDPs have recently been used as a modeling formalism in robotic planning \cite{Thrun05}. Formally, an MDP model is a tuple $\M = (S, s_0, A, \delta, r)$, 
where $S$ is a finite set of \emph{states}, 
$s_0\in S$ is an \emph{initial state}, 
$A$ is a set of \emph{actions},
$\delta: S\times A\times S \to [0,1]$ is a \emph{transition relation} mapping each state-action pair to a probability distribution over $S$,
and $r: S\times A \times S \to \mathbb{R}$ is a \emph{reward function}.
At each MDP state $s$, first an action $a \in A$ is chosen nondeterministically based on an MDP \emph{policy} $\sigma: S \to A$, 
then a success state $s'$ is chosen with the probability $\delta(s,a,s')$. Different methods for computing an optimal policy for an MDP model exist. However, our approach can be applied to all types of models and policy generation methods.

\startpara{Critical States}
Within an MDP, a critical state is one where the choice of action at the state greatly affects the MDP policy and performance \cite{Chen2020TowardsTR}. It can be defined through the impact that each possible choice at the state has on the current policy. If the difference between the greatest impact choice and the least impact choice is greater than some pre-defined threshold, $\alpha$, then the state is a critical state.
\begin{comment}
Formally, we define the set of critical states of an MDP model with the state space $S$ as
$$S_c = \{s\in S \ |\ (\lambda_s^{max} - \lambda_s^{min}) > \alpha\}$$
where $s$ is the state, $\lambda$ is the choice impact, and $\alpha$ is a user-defined threshold.
\end{comment}
For example, Figure \ref{fig:grid} has five critical states if the $\alpha$ is set to 0: 7, 12, 16, 17, 18. 

\startpara{Objective, Abstraction, Specificity, and Locality}
Objective refers to the objective that the system currently has to accomplish such as finding the shortest distance or most flexible path. In regard to explanations, the objective effects the reasoning that should be provided for the choices presented. According to \cite{VelosoVerbalization,DeyAbstraction}, ”Abstraction varies the vocabulary and concepts used in the narrative form concrete robot concepts, such as distances, speed, and time to abstract concepts, such as hallways, room, and landmarks.” Our system works with the four previously defined levels of abstraction: states/actions, times/distances, left/right, and landmarks. Locality ”varies the particular parts of the experience that the narration focuses on, from the global path to a local region or a landmark of interest” \cite{VelosoVerbalization,TomasonLocality}. We use the three levels of locality defined above with a global explanation presenting an explanation of all states, a regional explanation presets an explanation for several states, and a landmark explanation presenting an explanation of one state. Specificity ”varies the total number of concepts or words used” \cite{VelosoVerbalization,bohus2014directions}. For our system, varying the specificity varies the user-defined $\alpha$ when calculating the critical states present in the MDP. This effects where the user may update the system and receives an explanation. 
\begin{comment}
The base, or minimum $\alpha$, is 0 and includes all states. This allows the user to update at any state and receive information at any state. A higher $\alpha$ decreases the number of updatable and explainable states. The maximum $\alpha$ setting only allows updates and explanation at the most critical states in the route. The goal of a higher specificity is to lessen the cognitive burden that is placed on the user.
\end{comment}
\startpara{Verbalization Space}
The verbalization space is the collection of all possible route or explanation choices \cite{VelosoVerbalization}. This space can easily be expanded to contain metrics or reduced to limit explanation complexity. The potential verbalization space for our system is shown in Figure 2. 

\begin{figure}[ht]
     \centering
     \includegraphics[scale=0.3]{Figures/Table2.png}
     \caption{Verbalization Space for User Feedback System}
     \vspace{-10pt}
     \label{fig:table2}
 \end{figure}


==> draft/_Resolution.tex <==
Once we have detected a conflict, we present it to the user and ask them to resolve it by choosing between several recommendations generated by the system. By allowing the user to choose the resolution, we ensure the most  satisfactory and understandable set of realizable and valid preferences is given to the system.

\begin{comment}
\begin{algorithm}[]
\SetAlgoLined
\KwIn{Conflicts}
\KwOut{Recommendations}
 Recommendations=[]\\
 \For{Each Conflict}{
 \If{ChangeConflict}{
    Present Conflict to User\\
    Authenticate Preference Correctness\\
    \If{Preference Not Correct}{
    Update User Preferences\\
    \Return}}
\If{HardConflict}{
R = OptionGenerator\\(NewPreference,
CurrentPreferences);\\
Add R to Recommendations
}
\If{SoftConflict}{
N = OptionGenerator\\(NewPreference,CurrentPreferences);\\
Set NewPreference and Unset ConflictingPreference\\
C = OptionGenerator\\(ConflictingPreference,CurrentPreferences);}
 Create Pairs for NewPreference and C\\
 Create Pairs for ConflictingPreference and N\\
Add Pairs to Recommendations}
Remove Overlapping Recommendations\\
  \Return Recommendations
 \caption{Resolve Conflicts}
 \label{fig:resolveAlg}
\end{algorithm}

\begin{algorithm}[]
\SetAlgoLined
\KwIn{Preference,CurrentPreferences}
\KwOut{Options}
 O=[]\\
Generate Options For Preference Type\\
Remove Preference From Options\\
\For{Each Generated Option}{
\If{Option Still Conflicting}
{Remove Option}
Add Remaining Generated Options to O}

  \Return O
 \caption{Option Generator}
 \label{fig:resolveAlgHard}
\end{algorithm}
\end{comment}

\startpara{Resolving Soft Conflicts}
Soft conflicts only appear to be conflicts and do not need user resolution. We allow the system to move forward without pause.

\startpara{Resolving Hard and Unrealizable Conflicts}
However, both hard and unrealizable conflicts must be resolved by the user to maximize user satisfaction and understanding without fulfilling their total wants. Unrealizable conflicts are prioritized as their only resolution is a change in preference. We begin by generating the options for the conflicting preference and remove the options that still cause conflict with the user's other current preferences. The remaining options will be recommended to the user as possible choices for the preference. Yet, hard most often occur between preferences. So, we not only need to find the preference options that do not cause conflicts, but the pairs of options. We repeat the same process of generating all potential options and removing those that conflict with the other set preferences, but with all conflicting preferences to generate a list of viable pairs.

When all of the recommendations have been generated, we remove the overlapping recommendations, ordering them by likeness to the user's original new preference. This way, we suggest the user change the least preferences possible. An explanation is presented alongside the recommendations to increase user understanding of why the recommendation has been generated for them based on the conflict type and the preferences involved.
 
 \begin{example}
 Return to Example 3. We begin by authenticating the new preference and then generate recommendations for resolving the unrealizable conflict. We generate all possible options for the locality preference: only current position, only alleyways, only highways, and global, removing the only highways option since we know a conflict is present. The remaining options are recommended to the user as they cause no issues. The recommendation of global locality would be presented to the user first: "This option is closest to your new desired preference."
 The recommendation only the current position would be presented next: "This option lessens your section of interest." The recommendation of only alleyways would be presented last: "This option returns you to your original preference."
 
 Now, return to Example 4, a hard conflict.
 Starting with the locality preference, we generate all options: only current position, only alleyways, only highways, and global. We remove only highways and only alleyways since we know they conflict with the safest path objective. Then, we set the only alleyways locality preference and look at the possible objective preferences: minimize distance, minimize risk, and minimize distance and risk. We remove all options but minimize distance since we know the others conflict with our locality preference. Now, we generate all possible pairs of preferences: global and minimize risk ("closest to your new preference"), only current position and minimize risk ("has your new preference, but lessens your area of interest"), and only alleyways and minimize distance ("return to your old preferences"). The recommendations are presented in the order above and accompanied by their corresponding explanations.
 
 \end{example}


==> review.tex <==
Reviewer 2
The following content needs to be added:
1) The authors perform an evaluation based on 5-point Likert scale and show the average results in points. However they never state the concrete meaning of the numbers 1 to 5. Therefore, it can only be assumed that 5 is representing something like 'highly agree'. Please include at least the definition of 1 and 5 as defined in the questionnaire given to the MechTurk workers.
% I added a definition of the Likert scales for our study.

2) What is the chosen value to assume statistical significance and accept hypothesis H2? The p value mentioned in the manuscript is higher than the common p value of 0.05.
% I reran the experiments with a pvalue of 0.05. I also explained the meaning of a 0.05 pvalue.

The following content should be added to improve comprehensibility:
3) The samples of robot descriptions given in Section III-C are very good in general to enhance understanding, However, in the second example for the safest (green) rout, it is not clear how the shown explanations would differ to one of the shortest path objective. In particular, explanation 2) 'The robot moves along the corridor in the landmark' does not seem to reveal any information about turning left or right. The explanation does not seem to contain any information.
%Added a note that the white states in figure 2 are the corridor. It seems like the reviewer did not look back at the state names shown in the caption for figure 2.

4) It is very difficult to understand how changes in user preference occur/evolve. In the different strategies for conflict detection (Section III-E), it is mentioned that the system asks the user to update their preference. Why do the users have to update the preference. Isn't this done internally by the planing system?
% Added a sentence to soft, hard, and no conflict that users do not have to update their preferences unless they have made a mistake in preference input.

5) The previous question shows that it is in general not clear on the concrete learning of preferences takes place. There manuscript misses this description. This is maybe because the focus is on the evaluation of user preferences. However, as a result the manuscript misses essential information to understand all of the presented content.
% Described how preferences are originally learned in section 3-A as users select them from a drop-down.


Reviewer 3
1. The chosen environment is too simplistic to really gauge the merits of the system or the interactive question-answer approach.
% Need to motivate the choice of grid world?

2. The authors motivated the importance of robotic plan explanations by highlighting their effects on human users’ trust of robots and perceived system transparency.
However, the current study fails to demonstrate how personalized explanations affect these factors. For example, can personalized explanations increase trust when compared to standard explanations?
%Change trust to understanding and satisfaction.

3. If a robot designer wanted to use this system, how should they identify the template sentences that are required for the generation of explanations?
%Describe choice of template to match agent and environment needs by developer.

4. Definition of conflict is too simplistic and only considers a change in planning objective. How are conflicts along other factors solved? What if the choice in locality does not allow for a high abstraction of the plan explanation?
% Described that soft conflict causing elements only cause cosmetic changes to the explanation and thus cannot conflict one another.
%Changed abstraction to vocabulary.

Statistical analysis seems to be not well conducted:
5. In general it is not recommended to compare single likert-scale item (see “Four Years in Review: Statistical Practices of Likert Scales in Human-Robot Interaction Studies” for more detail)
%Cannot address this suggestion
% What I learned from the suggested paper:
% A Likert Scale is all of the questions that measure a metric. Each question in the scale is referred to as an item. Each item has a number of options within it. 
% The number of options for each item should be between 5 and 9
% You can include a neutral option on your item if you want to, but it is not required.
% There should be at least 4 items in any scale that is subjective (trust, understanding, satisfaction, etc.)
% They recommend no more than 40 questions in 1 survey
%We should use a scale that someone else has verified. However, if we make our own survey/scale we need to run a cronbach's alpha test to prove the consistency of our questions.
%We can preform a test on one item, but it is recommended not to and that we need to state if we do.
%If we do a significant number of test on the same metric (more than 3), we need apply Bonferonni correction or a similar test to make sure we didn't randomly find something significant.
%Anova is for normally distributed populations and Kruskal-wallis is for non-normally distributed populations. We can check this with a Shapiro-Wilk test and if its not normally distributed according to the Shapiro-Wilk it is recommended to run the Kruskal-wallis as to be safe. ANOVA and Kruskal-Wallis most often have the same results though. Friedman is the repeated measure version of Kruskal-Wallis.

6. Adhoc questionnaires with no measure of validity or reliability were used
% Cannot address this suggestion directly as we only have one question per metric
%I did state we have a single item per metric.

7. The authors didn’t check the basic assumptions required for an ANOVA test.Also, the authors seemed to forget that this is a repeated design experiment and an one-way ANOVA is not the appropriate test in this case.
% Ran and reported a Shapiro-Wilk. It indicated that the data was not normally distributed and we know this is a repeated measure study so we should use Friedman's Test to be safe as recommended by the paper.
%Checked the assumptions for Chi-squared and we meet them.

8.Were baseline and personalized explanations presented at the same time? Or oneafter the other one? Which one was presented first? The order of the conditions can potentially affect the participant’s answers and in general it is recommended to counterbalance all conditions to avoid an ordering confound effect.
% Described presentation of explanations together in a random order.

9.Formulation of hypothesis. Usually, the null hypothesis (no difference between samples) is stated first and the statistical analysis will aim at rejecting this hypothesis in favor of the alternative (there is a difference)
%Added the null hypotheses.

10.How was the quality of participants' answers assessed? It’s known that crowdsourcing answers might be noisy and contain outlier ratings.
%Added information about attention checks, removing outliers, and AMT user qualifications

11.Were participants briefed on the meaning of the different states in the environment?
%Indicated that users were told about possible agent movements and possible encounterable states.
